Personalizing Intervention Probabilities By Pooling

In many mobile health interventions, treatments should only be delivered in a particular context, for example when a user is currently stressed, walking or sedentary. Even in an optimal context, concerns about user burden can restrict which treatments are sent. To diffuse the treatment delivery over times when a user is in a desired context, it is critical to predict the future number of times the context will occur. The focus of this paper is on whether personalization can improve predictions in these settings. Though the variance between individuals' behavioral patterns suggest that personalization should be useful, the amount of individual-level data limits its capabilities. Thus, we investigate several methods which pool data across users to overcome these deficiencies and find that pooling lowers the overall error rate relative to both personalized and batch approaches.

==> related_work.tex <==
%!TEX root = ml4h_2018.tex
\section{Related Work} 
 Personalization has been a recent focus in healthcare prediction tasks. 
 Shoeb and Guttag \cite{shoeb2004} demonstrate that patient-specific classifiers are better able to infer the onset of epileptic seizures than population models. To classify affect and engagement among children with diabetes, Rudovic et al. \cite{rudovic2018} design a deep learning framework which can be fit to each individual, while still maintaining some population and subpopulation knowledge. Lopez and Picard \cite{lopez2017} propose a multi-task neural network for pain detection and Saeed and Trajanovski \cite{saeed2017} also propose a multi-task neural network approach, but for detecting stress. Each of these approaches is similar to ours in that the authors utilize between-subject pooling to improve personalization, however we have much higher data constraints in our setting. 

 
 %However, there is very little work on personalizing in the wild with the small groups of subjects which can be expected in active studies.    
